Towards Robust Knowledge Graph Embedding via Multi-task Reinforcement Learning

Nowadays, Knowledge graphs (KGs) have been playing a pivotal role in AI-related applications. Despite the large sizes, existing KGs are far from complete and comprehensive. In order to continuously enrich KGs, automatic knowledge construction and update mechanisms are usually utilized, which inevitably bring in plenty of noise. However, most existing knowledge graph embedding (KGE) methods assume that all the triple facts in KGs are correct, and project both entities and relations into a low-dimensional space without considering noise and knowledge conflicts. This will lead to low-quality and unreliable representations of KGs. To this end, in this paper, we propose a general multi-task reinforcement learning framework, which can greatly alleviate the noisy data problem. In our framework, we exploit reinforcement learning for choosing high-quality knowledge triples while filtering out the noisy ones. Also, in order to take full advantage of the correlations among semantically similar relations, the triple selection processes of similar relations are trained in a collective way with multi-task learning. Moreover, we extend popular KGE models TransE, DistMult, ConvE and RotatE with the proposed framework. Finally, the experimental validation shows that our approach is able to enhance existing KGE models and can provide more robust representations of KGs in noisy scenarios.

==> acknowledgements.tex <==
\section*{Acknowledgements}\label{sec:acknowledgements}
The research work is supported by the National Key Research and Development Program of China under Grant No. 2018YFB1004300, the National Natural Science Foundation of China under Grant No. U1836206, U1811461, 61773361, the Project of Youth Innovation Promotion Association CAS under Grant No. 2017146.

==> preliminaries.tex <==
\section{Preliminaries}\label{sec:preliminaries}
In this section, we briefly introduce the three models that we aim to extend in this paper.

\textbf{TransE}~\cite{bordes2013translating} assumes $\mathbf{h} + \mathbf{r} \approx  \mathbf{t}$ when ($h,r,t$) holds. The score function of TransE is defined as \begin{equation}\label{eq:transe_score}
f(h,r,t)=-\left \| \mathbf{h}+\mathbf{r}-\mathbf{t} \right \|_{L_{n}}.
\end{equation}
$L_n$ can be $L_1$ or $L_2$ norm, which is decided based on the model performance on the validation set. Positive triples are supposed to have higher scores than negative ones. 

\textbf{DistMult}~\cite{yang2015embedding} adopts a bilinear function to compute the scores of triples, which is defined as 
\begin{equation}\label{eq:distmult_score}
f(h,r, t) = \mathbf{h}^\top\mathbf{M}_r\mathbf{t},\vspace{0mm}
\end{equation}
where $\mathbf{M}_r$ is a relation-specific diagonal matrix, which represents the characteristics of a relation. Like triples in TransE, positive triples should have higher scores than negative ones in DistMult. 


\textbf{ConvE}~\cite{dettmers2018convolutional} models the interactions between input entities and relations by convolutional and fully-connected layers. Given ($h$, $r$, $t$) triples, ConvE first reshapes the embedding of $h$ and $r$ into 2D tensors, then computes the scores of knowledge triples based on the reshaped tensors. The score function of ConvE is defined as
\begin{equation}\label{eq:conve_score}
f(h, r, t)=g\left ( \text{vec}(g( [ \hat{\mathbf{h}};\hat{\mathbf{r}}  ]\ast \mathbf{\omega} ))\mathbf{W} \right )\mathbf{t},\vspace{0mm}
\end{equation} 
where $\hat{\mathbf{h}}$ and $\hat{\mathbf{r}}$ are 2D reshapings of $\mathbf{h}$ and $\mathbf{r}$: if $\mathbf{h}, \mathbf{r} \in \mathbb{R}^d$, then $\hat{\mathbf{h}}, \hat{\mathbf{r}} \in \mathbb{R}^{d_1 \times  d_2}$, where $d = d_1d_2$. $\mathbf{\omega}$ denotes a set of filters and $\ast$ denotes the convolution operator.
$\text{vec}(\cdot)$ is a vectorization function, $g$ denotes the ReLU function, and $\mathbf{W}$ is the weight matrix.
ConvE also assumes that positive triples have higher scores than negative ones.

The above three models are widely used to conduct the
KGE task and achieve competitive results on benchmarks.
